A Simple and Effective ASP-Based Tool for Enumerating Minimal Hitting Sets

The hitting set problem is a fundamental problem in computer science and mathematics. Given a family of sets over a universe of elements, a minimal hitting set is a subset-minimal collection of elements that intersects each set in the family. Enumerating all minimal hitting sets is crucial in various real-world applications. In this paper, we address the full enumeration of all minimal hitting sets for a given family of sets. We formulate the problem using Answer Set Programming (ASP) and leverage existing ASP solvers for efficient enumeration. We propose an ASP-based tool, MinHit-ASP, and our empirical evaluation shows that it effectively enumerates minimal hitting sets across benchmarks from diverse problem domains.

==> eptcsdata.tex <==
\providecommand{\firstpage}{238}
\providecommand{\publicationstatus}{M. Gebser, D. Inclezan, F. Ricca, M. Carro \& M. Truszczynski:\\
41st International Conference on Logic Programming (ICLP 2025)\\
EPTCS 439, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.439.17}{10.4204/EPTCS.439.17}}
\pdfoutput=1

